Bayesian identification of a projection-based Reduced Order Model for Computational Fluid Dynamics

In this paper we propose a Bayesian method as a numerical way to correct and stabilise projection-based reduced order models (ROM) in computational fluid dynamics problems. The approach is of hybrid type, and consists of the classical proper orthogonal decomposition driven Galerkin projection of the laminar part of the governing equations, and Bayesian identification of the correction term mimicking both the turbulence model and possible ROM-related instabilities given the full order data. In this manner the classical ROM approach is translated to the parameter identification problem on a set of nonlinear ordinary differential equations. Computationally the inverse problem is solved with the help of the Gauss-Markov-Kalman smoother in both ensemble and square-root polynomial chaos expansion forms. To reduce the dimension of the posterior space, a novel global variance based sensitivity analysis is proposed.

==> tex_files/preprocess.tex <==
\usepackage{lineno}
\makeatletter
\g@addto@macro\endfrontmatter{\enlargethispage{-2\baselineskip}}
\makeatother
\usepackage{bm}
\usepackage{amsfonts} 
\usepackage{multicol}
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{framed} % Framing content
\usepackage{multicol} % Multiple columns environment
\usepackage{tabularx}
\usepackage{tabulary}
\usepackage{siunitx}
\usepackage{caption}
\usepackage{float}
\usepackage{url} 
\usepackage{breakurl} 
\usepackage[breaklinks]{hyperref} 
%\usepackage{sfmath}
\renewcommand{\sectionautorefname}{\S}
\usepackage{subcaption}
\usepackage{xpatch}
\usepackage{nomencl} % Nomenclature package
\setlength{\nomitemsep}{-0.05cm}
\setlength{\nomlabelwidth}{1.5cm}
\renewcommand*{\nompreamble}{\footnotesize}
\makenomenclature
\makenomenclature 
\RequirePackage{ifthen}
\let\oldref\ref
\renewcommand{\ref}[1]{(\oldref{#1})}
\def\UrlBreaks{\do\/\do-}
%% Uncomment if you want the nomenclature on two columns 
% \setlength{\nomitemsep}{-\parskip} % Baseline skip between items
 
% \renewcommand*\nompreamble{\begin{multicols}{2}}
% \renewcommand*\nompostamble{\end{multicols}}
% \newcolumntype{Y}{>{\centering\arraybackslash}X}  
\usepackage{amssymb}
\providecommand{\norm}[1]{\lVert#1\rVert}
\newcommand{\ten}[1]{\mathsfbfit{#1}}
\newcommand{\vc}[1]{\mathbfit{#1}}
\newcommand{\ltwonorm}[1]{\langle #1 \rangle_{L^2(\mathcal{G})}}
\newdefinition{rmk}{Remark}
%%

\DeclareMathOperator{\spn}{span}
\DeclareMathAlphabet\mathbfcal{OMS}{cmsy}{b}{n}

\xpatchcmd{\thenomenclature}{%
  \section*{\nomname}% Look for `\section*... etc.
}{% Replace it by 'nothing'
}{\typeout{Success}}{\typeout{Failure}}

%\renewcommand{\nomname}{Abbreviations and Symbols}

\usepackage{ifthen}
\renewcommand{\nomgroup}[1]{%
  \ifthenelse{\equal{#1}{A}}{\item[\textbf{Abbreviations}]}{%
    \ifthenelse{\equal{#1}{G}}{\item[\textbf{Symbols}]}{%
      \ifthenelse{\equal{#1}{C}}{\item[\textbf{Abbreviations}]}{%
        \ifthenelse{\equal{#1}{S}}{\item[\textbf{Subscripts}]}{%
          \ifthenelse{\equal{#1}{Z}}{\item[\textbf{Mathematical Symbols}]}{}
        }% matches mathematical symbols
      }% matches Subscripts
    }% matches Abbreviations
  }% matches Greek Symbols
}% matches Roman Symbols


\journal{Computers \& Fluids}  

%%%%%%%%%%%%%%%%%%%%%%%
%% Elsevier bibliography styles
%%%%%%%%%%%%%%%%%%%%%%%
%% To change the style, put a % in front of the second line of the current style and
%% remove the % from the second line of the style you would like to use.
%%%%%%%%%%%%%%%%%%%%%%%

%% Numbered
%\bibliographystyle{model1-num-names} 

%% Numbered without titles
%\bibliographystyle{model1a-num-names}

%% Harvard
%\bibliographystyle{model2-names.bst}\biboptions{authoryear}

%% Vancouver numbered
%\usepackage{numcompress}\bibliographystyle{model3-num-names}

%% Vancouver name/year
%\usepackage{numcompress}\bibliographystyle{model4-names}\biboptions{authoryear}

%% APA style
%\bibliographystyle{model5-names}\biboptions{authoryear}

%% AMA style
%\usepackage{sty/numcompress}\bibliographystyle{model6-num-names}

%% `Elsevier LaTeX' style
\bibliographystyle{bst/elsarticle-num}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> tex_files/preprocess_arxiv.tex <==
\usepackage{lineno}
\usepackage{bm}
\usepackage{amsfonts} 
\usepackage{multicol}
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{framed} % Framing content
\usepackage{multicol} % Multiple columns environment
\usepackage{tabularx}
\usepackage{tabulary}
\usepackage{siunitx}
\usepackage{caption}
\usepackage{float}
\usepackage{url} 
\usepackage{breakurl} 
\usepackage[breaklinks]{hyperref} 
%\usepackage{sfmath}
\renewcommand{\sectionautorefname}{\S}
\usepackage{subcaption}
\usepackage{xpatch}
\usepackage{nomencl} % Nomenclature package
\setlength{\nomitemsep}{-0.05cm}
\setlength{\nomlabelwidth}{1.5cm}
\renewcommand*{\nompreamble}{\footnotesize}
\makenomenclature
\makenomenclature 
\RequirePackage{ifthen}
\let\oldref\ref
\renewcommand{\ref}[1]{(\oldref{#1})}
\def\UrlBreaks{\do\/\do-}
%% Uncomment if you want the nomenclature on two columns 
% \setlength{\nomitemsep}{-\parskip} % Baseline skip between items
 
% \renewcommand*\nompreamble{\begin{multicols}{2}}
% \renewcommand*\nompostamble{\end{multicols}}
% \newcolumntype{Y}{>{\centering\arraybackslash}X}  
\usepackage{amssymb}
\providecommand{\norm}[1]{\lVert#1\rVert}
\newcommand{\ten}[1]{\mathsfbfit{#1}}
\newcommand{\vc}[1]{\mathbfit{#1}}
\newcommand{\ltwonorm}[1]{\langle #1 \rangle_{L^2(\mathcal{G})}}
%%

\DeclareMathOperator{\spn}{span}
\DeclareMathAlphabet\mathbfcal{OMS}{cmsy}{b}{n}

\xpatchcmd{\thenomenclature}{%
  \section*{\nomname}% Look for `\section*... etc.
}{% Replace it by 'nothing'
}{\typeout{Success}}{\typeout{Failure}}

%\renewcommand{\nomname}{Abbreviations and Symbols}

\usepackage{ifthen}
\renewcommand{\nomgroup}[1]{%
  \ifthenelse{\equal{#1}{A}}{\item[\textbf{Abbreviations}]}{%
    \ifthenelse{\equal{#1}{G}}{\item[\textbf{Symbols}]}{%
      \ifthenelse{\equal{#1}{C}}{\item[\textbf{Abbreviations}]}{%
        \ifthenelse{\equal{#1}{S}}{\item[\textbf{Subscripts}]}{%
          \ifthenelse{\equal{#1}{Z}}{\item[\textbf{Mathematical Symbols}]}{}
        }% matches mathematical symbols
      }% matches Subscripts
    }% matches Abbreviations
  }% matches Greek Symbols
}% matches Roman Symbols

%%%%%%%%%%%%%%%%%%%%%%%
%% Elsevier bibliography styles
%%%%%%%%%%%%%%%%%%%%%%%
%% To change the style, put a % in front of the second line of the current style and
%% remove the % from the second line of the style you would like to use.
%%%%%%%%%%%%%%%%%%%%%%%

%% Numbered
%\bibliographystyle{model1-num-names} 

%% Numbered without titles
%\bibliographystyle{model1a-num-names}

%% Harvard
%\bibliographystyle{model2-names.bst}\biboptions{authoryear}

%% Vancouver numbered
%\usepackage{numcompress}\bibliographystyle{model3-num-names}

%% Vancouver name/year
%\usepackage{numcompress}\bibliographystyle{model4-names}\biboptions{authoryear}

%% APA style
%\bibliographystyle{model5-names}\biboptions{authoryear}

%% AMA style
%\usepackage{sty/numcompress}\bibliographystyle{model6-num-names}

%% `Elsevier LaTeX' style
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
